Coherent Emission Mechanisms in Astrophysical Plasmas

Three known examples of coherent emission in radio astronomical sources are reviewed: plasma emission, electron cyclotron maser emission (ECME) and pulsar radio emission.

==> Repy.tex <==
The only point raised by the referee concerned labelling on the axes of figure 16. This has been corrected in the revised manuscript
